Lower Bounds for Alternating Online State Complexity

The notion of Online State Complexity, introduced by Karp in 1967, quantifies the amount of states required to solve a given problem using an online algorithm, which is represented by a deterministic machine scanning the input from left to right in one pass. In this paper, we extend the setting to alternating machines as introduced by Chandra, Kozen and Stockmeyer in 1976: such machines run independent passes scanning the input from left to right and gather their answers through boolean combinations. We devise a lower bound technique relying on boundedly generated lattices of languages, and give two applications of this technique. The first is a hierarchy theorem , stating that the polynomial hierarchy of alternating online state complexity is infinite, and the second is a linear lower bound on the alternating online state complexity of the prime numbers written in binary. This second result strengthens a result of Hartmanis and Shank from 1968, which implies an exponentially worse lower bound for the same model.

==> det.tex <==
\begin{theorem}
The polynomial hierarchy of deterministic online space complexity is infinite.
\end{theorem}

For the case of deterministic automata, lower bounds are obtained by considering the number of left quotients for each order,
as suggested by Proposition~\ref{prop:lower_bound_det}.

Let $\ell \ge 1$.

Denote 
$$\Eq_\ell = \set{w \in \set{a,a_1,\ldots,a_\ell}^* \mid \exists i \in \set{1,\ldots,\ell}, |w|_a = |w|_{a_i}}.$$

\begin{proposition}
The following properties hold for all $\ell \ge 1$:
\begin{itemize}
	\item $\Eq_\ell$ is in $\Det{O(n^{\ell + 1})}$,
	\item $\Eq_\ell$ is not in $\Det{O(n^\ell)}$,
	\item $\Eq_\ell$ is in $\ND{O(n^2)}$.
\end{itemize}
\end{proposition}

\begin{proof}\hfill
\begin{itemize}
	\item We construct a deterministic automaton recognising $\Eq_\ell$ of size $O(n^{\ell + 1})$,
	generalising the construction given above for $\Eq_3$.

Formally, the set of states is $\Z^{\ell}$, the initial state is the null vector, the letter $a$ acts as $(+1,\ldots,+1)$,
and the letter $a_i$ as $(0,\ldots,0,-1,0,\ldots,0)$ where the $-1$ is on position $i$.
The set of accepting states is 
$$\set{(c_1,\ldots,c_\ell) \mid \exists i \in \set{1,\ldots,\ell}, c_i = 0}.$$
After reading the word $w$, the automaton is in the state 
$$(|w|_a - |w|_{a_1}, |w|_a - |w|_{a_2},\ldots, |w|_a - |w|_{a_\ell}),$$
implying that it has size $O(n^{\ell + 1})$.

	\item We now prove that $\Eq_\ell$ is not in $\Det{O(n^\ell)}$.

Note that $u^{-1} \Eq_\ell = v^{-1} \Eq_\ell$ if, and only if, $u$ and $v$ have the same number of occurrences of each letter.
For words on length $n$, this describes $\binom{n+\ell}{\ell}$ different classes,
which as a function of $n$ is equivalent to $n^{\ell}$.
It follows that the number of left quotients of $\Eq_\ell$ of order $n$ is equivalent to $n^{\ell + 1}$.
This concludes.

	\item We construct a non-deterministic automaton recognising $\Eq_\ell$ of quadratic size.
	It starts by guessing a letter $a_i$, and uses one counter to store the value $w_{|a|} - w_{|a_i|}$.

Formally, the set of states is $\set{1,\ldots,\ell} \times \Z$ 
and the initial and accepting states are $\set{1,\ldots,\ell} \times \set{0}$\footnote{In our definition we did not allow for several initial states. 
This slight abuse could be avoided, it is here for the sake of readability.}.
The transitions are:
$$\begin{array}{l}
\delta((i,n),a) = (i,n+1) \\
\delta((i,n),a_i) = (i,n-1) \\
\delta((i,n),a_j) = (i,n)
\end{array}$$
\end{itemize}
\qed\end{proof}


==> left_quotients.tex <==
We present a first technique to give lower bounds on the online space complexity,
relying on the notion of left quotients.

Let $w$ be a finite word, define its left quotient with respect to $L$ by
$$w^{-1} L = \set{u \mid w u \in L}.$$

A well known result from automata theory states that the existence of a minimal deterministic automaton, called the \textit{syntactic automaton}, whose states of the left quotients.

This construction extends \textit{mutatis mutandis} when dropping the assumption that the automaton has finitely many states, \textit{i.e.} going from deterministic automata to machines as we defined them.
The statement, however, is more involved, and gives precise lower bounds 
on the online space complexity of the language.

Formally, consider a language $L$, we define the syntactic machine of $L$, denoted $\M_L$,
as follows. 
We define the set of states as the set of all left quotients: $\set{w^{-1} L \mid w \in A^*}$.
The initial state is $\varepsilon^{-1} L$, and the transition function is defined by
$\delta(w^{-1} L, a) = (wa)^{-1} L$.
Finally, the set of accepting states is $\set{w^{-1} L \mid w \in L}$.

Denote $s_L$ the size of the syntactic machine of $L$.

\begin{theorem}\leavevmode
\label{thm:lower_bound_left_quotients}
\begin{itemize}
	\item $\M_L$ recognises $L$, so $L \in \Dyn(s_L)$,
	\item for all $f$, if $L \in \Dyn(f)$, then $f \ge s_L$.
\end{itemize}
\end{theorem}

Note that the implies the existence of a minimal function $f$ such that $L \in \Dyn(f)$;
in other words $L \in \Dyn(f)$ if, and only if, $f \ge s_L$.
This was not clear a priori, because the order on functions is partial.

The first item is routinely proved, as in the case of automata.
For the second item, assume towards contradiction that there exists $f$ such that $L \in \Dyn(f)$
and $f \not\ge s_L$, \textit{i.e.} there exists $n$ such that $f(n) < s_L(n)$.
Consider a machine $\M$ recognising $L$ of size $f$.
Since $f(n) < s_L(n)$, there exists two words $u$ and $v$ of length $n$
such that $u^{-1} L \neq v^{-1} L$ but $c(u) = c(v)$, \textit{i.e.} in $\M$ the words $u$ and $v$ lead to the same state.
The left quotients $u^{-1} L \neq v^{-1} L$ being different, there exists a word $w$ such that 
$uw \in L$ and $vw \notin L$, or the other way around.
But $c(uw) = c(vw)$ since $\M$ is deterministic, so this state must be both accepting and rejecting, contradiction.

The view using left quotients is very powerful, as it gives the exact online space complexity of a language. 
However, it is sometimes hard to deal with, as it may involve complicated word combinatorics.
We illustrate it on some of the examples introduced in subsection~\ref{subsec:examples}.

To prove for instance that $L$ has an online space complexity at least linear using this technique,
one has to exhibit, for infinitely many $n$, 
a family of linearly many words (\textit{i.e.}, at least $a n$ words, for some constant $a$) of length at most $n$ that induce pairwise distinct left quotients.

\begin{example}\leavevmode
\begin{itemize}
	\item Fix $n$. The words $a^{n+k} b^{n-k}$, for $0 \le k \le n$, have length $2n$ and all induce pairwise distinct left quotients,
	since $a^{n+k} b^{n-k} \cdot b^p \in \Maj_2$ if, and only if, $p < 2k$.
	It follows from Theorem~\ref{thm:lower_bound_left_quotients} that $\Maj_2$ has linear online space complexity.
	\item Fix $n$. The words $a^{2n-p-q} b^p c^q$, for $0 \le p,q \le n$, have length $2n$ and all induce pairwise distinct left quotients,
	since $a^{2n-p-q} b^p c^q \cdot a^{k+\ell} b^{2n-k} c^{2n-\ell} \in \Eq$ if, and only if, $k = p$ and $\ell = q$.
	It follows from Theorem~\ref{thm:lower_bound_left_quotients} that $\Eq$ has quadratic online space complexity.
\end{itemize}
\end{example}

==> non-det.tex <==
\begin{theorem}
The polynomial hierarchy of non-deterministic online space complexity is infinite.
\end{theorem}

The lower bounds will be achieved using the Rank Method.
As we are here interested in non-deterministic automata, we specialise Theorem~\ref{thm:rank_method},
in the following corollary.

\begin{corollary}
Let $L$ in $\ND{f}$ and $n \in \N$. 
The rank of the lattice generated by the left quotients of $L$ of order $n$ is at most $2^{f(n)} - 1$.
\end{corollary}

Let $\ell \ge 1$.

Denote 
$$\NotEq_\ell = \set{u \sharp u_1 \sharp u_2 \sharp \cdots \sharp u_\ell 
\left|
\begin{array}{c}
u,u_1,\ldots,u_\ell \in \set{0,1}^*, \\
\forall i \in \set{1,\ldots,\ell}, u \neq u_i
\end{array}
\right.}.$$

\begin{proposition}
The following properties hold for all $\ell \ge 1$:
\begin{itemize}
	\item $\NotEq_\ell$ is in $\ND{O(n^{\ell+1})}$,
	\item $\NotEq_\ell$ is not in $\ND{O(n^\ell)}$,
	\item $\NotEq_\ell$ is in $\Alt{O(n^2)}$.
\end{itemize}
\end{proposition}

\begin{proof}\hfill
\begin{itemize}
	\item We construct a non-deterministic automaton recognising $\NotEq_\ell$ of size $O(n^{\ell+1})$,
	generalising the construction given above for $\NotEq$.
	
%The automaton has two consecutive phases:
%\begin{enumerate}
%	\item First, a non-deterministic phase while reading $u$.
%	The automaton guesses position, and stores it together with the letter of $u$ at this position.
%	The states passed onto the third phase are of the form $(j,a,i)$, where $j$ if the position guessed, $a$ is the letter of $u$ at position $j$,
%	and $i$ the number guessed in the first phase.
%	\item Second, a deterministic phase while reading $\sharp u_1 \sharp u_2 \sharp \cdots \sharp u_k$.
%	The state $(j,a,i)$ checks whether in $u_i$, the position $j$ carries a letter different from $a$.
%	The localisation of the $u_i$ is achieving by decrementing the number $i$ by one each time a letter $\sharp$ is read.
%	While in the corresponding $u_i$, the localisation of the position $j$ in $u_i$ as achieved by decrementing one position at a time.
%\end{enumerate}

%Formally, \mynote{TO DO}
%the set of states is $\Z^{\ell}$, the initial state is the null vector, the letter $a$ acts as $(+1,\ldots,+1)$,
%and the letter $a_i$ as $(0,\ldots,0,-1,0,\ldots,0)$ where the $-1$ is on position $i$.
%The set of accepting states is 
%$$\set{(c_1,\ldots,c_\ell) \mid \exists i \in \set{1,\ldots,\ell}, c_i = 0}.$$
%After reading the word $w$, the automaton is in the state 
%$$(|w|_a - |w|_{a_1}, |w|_a - |w|_{a_2},\ldots, |w|_a - |w|_{a_\ell}),$$
%implying that it has size $O(n^{\ell})$.

	\item We now show the lower bound.

We prove that for all $n$, the rank of the family of left quotients of $L$ of order $n$ is at least $\binom{n}{\ell}$,
which as a function of $n$ is equivalent to $n^\ell$.
It follows from Proposition~\ref{prop:lower_bound_nondet} that $L$ is not in $\ND{O(n^{\ell-1})}$.

Consider the set of words of length $n$ 

	\item We construct an alternating automaton recognising $\NotEq_\ell$ of quadratic size.
%	It starts by guessing a letter $a_i$, and uses one counter to store the value $w_{|a|} - w_{|a_i|}$.

%Formally, the set of states is $\set{1,\ldots,\ell} \times \Z^{\ell}$ 
%and the initial and final states are $\set{1,\ldots,\ell} \times \set{0}$\footnote{In our definition we did not allow for several initial states. 
%This slight abuse could be avoided, it is here for the sake of readability.}.
%The transitions are:
%$$\begin{cases}
%\delta((i,n),a) = (i,n+1) \\
%\delta((i,n),a_i) = (i,n-1) \\
%\delta((i,n),a_j) = (i,n)
%\end{cases}$$
\end{itemize}
\qed\end{proof}

